High-frequency shape recovery from shading by CNN and domain adaptation

Importance of structured-light based one-shot scanning technique is increasing because of its simple system configuration and ability of capturing moving objects. One severe limitation of the technique is that it can capture only sparse shape, but not high frequency shapes, because certain area of projection pattern is required to encode spatial information. In this paper, we propose a technique to recover high-frequency shapes by using shading information, which is captured by one-shot RGB-D sensor based on structured light with single camera. Since color image comprises shading information of object surface, high-frequency shapes can be recovered by shape from shading techniques. Although multiple images with different lighting positions are required for shape from shading techniques, we propose a learning based approach to recover shape from a single image. In addition, to overcome the problem of preparing sufficient amount of data for training, we propose a new data augmentation method for high-frequency shapes using synthetic data and domain adaptation. Experimental results are shown to confirm the effectiveness of the proposed method.

==> tex/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

We have proposed a method based on the learning of shading to recover the high-frequency shapes lost in the low-frequency shapes obtained in the measurements.
Since it is difficult to construct a large dataset measured in the real environment, we train the model by a dataset of synthetic images and adapt its domain for real-world images.
It is confirmed that the high-frequency shape of the object in the real environment can be reconstructed.
On the other hand, we evaluate the shape by normalizing the depth to remove scale indeterminacy and bas relief ambiguity.
% the bas relief ambiguity of the shading information under a single illumination led to the estimation of the shape of the unevenness contrary to reality, or the accuracy of the absolute distance was not improved in some cases.
%
In future studies, we will investigate methods to eliminate bas relief ambiguity and to create synthetic data that can be used to obtain images close to real-world images.
    \vspace{-0.2cm}


==> tex/experiment.tex <==
\section{Experiment} \label{sec:experiment}
% In addition to the synthetic data, we prepared 6 types of real objects taken in the real environment: cardboards with three different high-frequency shapes and the other three objects with more complex surface shapes.
% Of the three cardboard boxes A, B, and C, 40 data taken at A are used as training data and 16 data taken at B and C are used as test data.

% \subsection{Training}
% Of the 200 simulation data, 40 data were used as test data, and 48 of the remaining 160, or 30\% of the data, were used as validation data, resulting in 92 pieces of training data.
% The $1200\times1200$ resolution data is clipped into $120\times120$ resolution patches and entered into the network.
% The model was trained at 400 epochs and evaluated with the model at the point of lowest validation loss.

% Image data augmentation (shift, rotation, and zoom) was used to expand the training dataset in order to improve the performance.
% The data augmentation randomly shifts the original images up to 20\% of image size, rotates between 0 to 90 degrees, and zooms from 80\% to 120\%.
% To confirm the validity of the data augmentation, we also learned without it and compared the models.
\subsection{Datasets and training}
We prepared 6 types of real objects taken in the real environment: cardboards with three different high-frequency shapes (A, B, and C) and the other three objects with more complex surface shapes (\textit{shoes}, \textit{mesh}, and \textit{basket}).
Of the three cardboards A, B, and C, 16 data taken at A are used as training data and 16 data taken at B and C are used as test data.

Of the 200 synthesized data, 40 data were used as test data, and 48 of the remaining 160, or 30\% of the data, were used as validation data, resulting in 92 pieces of training data.
No additional augmentation is employed for training.
The $1200\times1200$ resolution data is clipped into $120\times120$ resolution patches and entered into the network.
The model was trained at 400 epochs and evaluated with the model at the point of lowest validation loss.

In domain adaptation, synthetic data is used to train sufficient epochs until convergence, and then fine-tuning is performed using real-world data (cardboard-A).

The training and validation loss for fine-tune is shown in \fref{fig:result_train_loss}.
In the first epoch of the fine-tune stage, both loss values are high, but it decreases rapidly in the first few epochs.
In the case of training loss, the training loss continues to decrease, whereas the validation loss starts to increase after about 80 epochs.
We utilized the model at the validation loss is at its minimum for fine-tune.
\begin{figure}[t]
    \centering
    \includegraphics[width=1 \linewidth]{figs/Result/Training/loss_graph-ft.pdf}
    \caption{Training and validation loss of fine-tune method.}
    \label{fig:result_train_loss}
\end{figure}

\subsection{Evaluation method}
To confirm that the output results of the network recovered the more correct shape than input depth, the Root Mean Square Error (RMSE) with ground-truth (GT) is calculated and evaluated.
Since we use shading to estimate the shape of the object, scale and indeterminacy of convexity (known as bas relief ambiguity~\cite{belhumeur1999bas}) can be a problem.
Due to this problems, the scale of the output is adjusted by GT, in order to confirm that the surface shape is adequately estimated.
In scaling the output, we compute the mean and variance of the GT and output for a $7\times7$ patch around a pixel and normalize the output.
% In scaling the output, the output is divided into $12\times12$ patches and the average and variance of the patches are adjusted to match the GT.
% In correcting the inversion of the unevenness, where the error of the output is greater than the threshold of 1 mm, the smaller one is adopted compared to the inverted output.

% In addition to the test data created in the simulator, actual data taken in the real environment were also prepared for the evaluation.
% Three types of cardboard with high-frequency shapes similar to the synthesized data used in the training were prepared and captured in eight different poses each.
% One of the three types of cardboard is for fine-tuning, which will be explained later in the \secref{discuss}.
% Additionally, three objects with various shapes (a basket, a shoe and a mesh) were captured in three different poses.

\subsection{Validation on real-world objects}
We validate our method by reconstructing the real-world objects.
The reconstructed depth of \textit{cardboard} by fine-tune model is shown in \fref{fig:result_3high-freq}.
The model is fine-tuned using a \textit{cardboard} (A), but the width and height of the test \textit{cardboard} (B, C) are different.
The upper row shows the distance and the lower row shows the error from GT.
In the proposed method, the high-frequency shape, which was lost in the low-resolution depth, is reconstructed.
The effect of the restoration can be confirmed more clearly in the 3-D reconstruction (\fref{fig:3d_shapes_cardboard}), where shading according to the normal direction is visualized.

\begin{figure}[t]
    \centering
    \subfigure[]{\includegraphics[width=0.97 \linewidth]{figs/Result/CMap/result_board-B.png}}
    \subfigure[]{\includegraphics[width=0.97 \linewidth]{figs/Result/CMap/result_board-C.png}}
   \caption{Reconstructed depth by fine-tune model: (a) cardboard B, and (b) cardboard C.
   The top row is the depth and the bottom row is the shading image and the error from the GT. It is clearly shown that error of high frequency pattern is largely decreased.}
    \label{fig:result_3high-freq}
\end{figure}
\begin{figure}[t]
    \centering
    \subfigure[]{\includegraphics[width=0.75\linewidth]{figs/Result/3DPoint/3d_boardC_gt.png}}
    \subfigure[]{\includegraphics[width=0.75\linewidth]{figs/Result/3DPoint/3d_boardC_rec.png}}
    \subfigure[]{\includegraphics[width=0.75\linewidth]{figs/Result/3DPoint/3d_boardC_pred.png}}
    \caption{3D reconstruction of cardboard-C. (a) GT. (b) Low-resolution. (c) Proposed.}
    \label{fig:3d_shapes_cardboard}
\end{figure}

The result for more complex shapes (\textit{shoes}, \textit{mesh}, and \textit{basket}) are shown in \fref{fig:result_2real}.
The shape of \textit{shoes} (\fref{fig:result_2real}(a)) is a mixture of one-dimensional and two-dimensional waves, and the shape of mesh (\fref{fig:result_2real}(b)) is basically two-dimensional wave.
The reconstructed shapes of the proposed method are more accurate than that of low-resolution.
In the \textit{basket} (\fref{fig:result_2real}(c)), although there are many holes and specular reflections in the shading images, the proposed method robustly restores the high-frequency shape.
3-D reconstruction of \textit{shoes} is shown in \fref{fig:3d_shoes}.
A flat area and high-frequency waves are accurately reconstructed.
The noisy area on the left is probably due to the fact that it was partially occluded from the point of view.
\begin{figure}[t]
    \centering
    % \subfigure[]{\includegraphics[width=0.97 \linewidth]{figs/Result/CMap/result_shoes.png}}
    \subfigure[]{\includegraphics[width=0.9 \linewidth]{figs/Result/CMap/result_shoes_large.jpg}}
    \subfigure[]{\includegraphics[width=0.9 \linewidth]{figs/Result/CMap/result_mesh.png}}
    \subfigure[]{\includegraphics[width=0.9 \linewidth]{figs/Result/CMap/result_basket.png}}
   \caption{Reconstructed depth of complex shapes: (a) shoes. (b) mesh. (c)basket.}
    \label{fig:result_2real}
\end{figure}
\begin{figure}[t]
    \centering
    \subfigure[]{\includegraphics[width=0.75\linewidth]{figs/Result/3DPoint/3d_shoes_gt.png}}
    \subfigure[]{\includegraphics[width=0.75\linewidth]{figs/Result/3DPoint/3d_shoes_rec.png}}
    \subfigure[]{\includegraphics[width=0.75\linewidth]{figs/Result/3DPoint/3d_shoes_pred.png}}
    \caption{3D reconstruction of shoes. (a) GT. (b) Low-resolution. (c) Proposed.}
    \label{fig:3d_shoes}
\end{figure}

\subsection{Evaluation on domain adaptation}
% training: synthesized, fine-tune, cardboard only
% inference: synthesized, cardboard, real-world objects
In this experiment, we confirm the effect of the domain adaptation we propose.
We compare the accuracy of depth estimation between models trained with synthetic data, a small number of real-world data and the fine-tune model.
The fine-tune is performed using the synthetic and real-world datasets for the other trained models.

The RMSE of depth estimation on the test data of the various domain is shown in \fref{fig:result_domain_adaptation}.
Example of test data is shown in \fref{fig:comp_domain_adaptation}.
For the synthetic data, the model trained with the same domain outperforms other models.
Beside the model trained with the real-world data works poorly in the synthetic domain, we find that the fine-tune model also reduces the ability to estimate synthetic data as a result of additional training with real-world data.

For the \textit{cardboard}, models trained on only synthetic data performed worse than other models trained with real-world data.
The model trained with real-world data is trained with \textit{cardboard} (A), so that the domain of the data is the same, but the pitch and height of the waves are different. 
The model can also estimate other \textit{cardboard} data with relatively small errors, but it does not match the accuracy of the fine-tune model.
This result suggests that the fine-tune model covers the variation in the test data thanks to the variation of the synthetic data.

For various other real-world data, the fine-tune model consistently estimates with small errors, showing that this domain adaptation is useful for estimating a wide variety of real-world data.
The model trained with real-world data works as good as fine-tune on \textit{shoes} and \textit{basket}, but not on \textit{mesh}.
It suggests the the model is over-fitted to the \textit{cardboard} and does not handles the real-world data which has different features.
\begin{figure}[t]
    \centering
    \includegraphics[width=1 \linewidth]{figs/Result/DomainAdaptation/rmse_avg_domain.pdf}
    \caption{Effect of training dataset on depth estimation.}
    \label{fig:result_domain_adaptation}
\end{figure}
\begin{figure}[t]
    \centering
    \subfigure[]{\includegraphics[width=1 \linewidth]{figs/Result/DomainAdaptation/comp_adap_cardboard.pdf}}
    \subfigure[]{\includegraphics[width=1 \linewidth]{figs/Result/DomainAdaptation/comp_adap_mesh.pdf}}
    \caption{Example of estimated depth by different models. (a) cardboard. (b) mesh.}
    \label{fig:comp_domain_adaptation}
\end{figure}

% The results of the test data created by the simulator are shown in \figref{result_simu}.
% As you can see from the error map, the shape of the output is close to the real shape.
% We confirm that the network is estimating the correct shape by comparing it to the input depth, where the high-frequency shape is not recovered.
% The \figref{rmse_avg_simu} shows the mean of the RMSE on the 40 test data compared to the depth of the input, Low-res.
% On average, the RMSE was 1.2 mm smaller in the 40 tests of synthetic data.
% The results show that the network is able to learn the unevenness of the synthetic data.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1 \linewidth]{figs/Experiment/result_simu_1wave.png}
%     \caption{The top row is the depth and the bottom row is the shading image and the error from the GT.}
%     \label{fig:result_simu}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7 \linewidth]{figs/Experiment/rmse_avg_simu.png}
%     \caption{On average, the RMSE was 1.18 mm smaller in the 40 tests of synthetic data.}
%     \label{fig:rmse_avg_simu}
% \end{figure}

\subsection{Dependency on degree of freedom (DoF) of synthesized data}
% training: 1-wave + FT, 2-waves + FT
% inference: cardboard, shoes, mesh, basket
Synthesized data is generated by rendering the shape composed of the multiple waves of different directions.
The DoF of the synthesized shape, i.e., the number of waves used, is expected to lead to differences in estimation accuracy for shapes with different features.
We compare the estimation accuracy of models trained on datasets with different DoF on real-world data.

The result is shown in \fref{fig:result_dof_synthetic}.
For the \textit{cardboard}, both models successfully reconstructs the depth with high accuracy.
Since the \textit{shoes} consist of a 1-wave and 2-waves structure, both training sets are equally accurate.
For the \textit{mesh}, the 2-waves dataset is more accurate because it is composed of fibers in two different directions.
For the \textit{basket}, 1-wave dataset is more accurate, while it appears to have a similar structure to \textit{mesh}.
However, since baskets are made up of wavy, flat fibers (\fref{fig:dof_3d_basket}), they are considered to be close to 1-wave in reality.

\begin{figure}[t]
    \centering
    \includegraphics[width=1 \linewidth]{figs/Result/DoF/rmse_avg_waves.pdf}
    \caption{Effect of synthetic data's DoF.}
    \label{fig:result_dof_synthetic}
\end{figure}
\begin{figure}[t]
    \centering
    \subfigure[GT.]{\includegraphics[width=0.49 \linewidth]{figs/Result/DoF/3d_basket_gt.png}}
    \subfigure[Fine-tune.]{\includegraphics[width=0.49 \linewidth]{figs/Result/DoF/3d_basket_pred.png}}
    \caption{3D reconstruction of basket.}
    \label{fig:dof_3d_basket}
\end{figure}

\subsection{Comparison with other methods}
% training: 2-waves + FT, Super-resolution by guided-filter
% inference: cardboard, shoes, mesh, basket

We further compared to one of the state-of-the-art depth super-resolution technique, \cite{Lutio2019}. For a clipped $255\times255$ area, the shading image is input as a guide image. We also gave a low-frequency distance image down-sampled to 1/3 (roughly consistent with the number of samples in our measurement method) as a low-resolution depth. The result is shown in \figref{compare_guide}. While \cite{Lutio2019} uses the shading image as a guide image to slightly restore the high-frequency shape, the proposed method succeeds in restoring it to a greater degree. One reason could be that \cite{Lutio2019} is an unsupervised method and failed to relate shading to normal direction.

\begin{figure}[t]
    \centering
    % \subfigure[]{\includegraphics[width=0.5\linewidth]{figs/Experiment/comp_guide_1.pdf}}
    \subfigure[]{\includegraphics[width=1\linewidth]{figs/Result/Guide/rmse_avg_vs-guided.pdf}}
    \subfigure[]{\includegraphics[width=1\linewidth]{figs/Result/Guide/vs-guided_boardC.jpg}}
    \caption{Comparison of shape recovery errors with \cite{Lutio2019}. The proposed method accurately recovers the high-frequency geometry in both (a)  the numerical evaluation and (b) the error map.}
    \label{fig:compare_guide}
\end{figure}

% \subsection{Discussion}
% \label{sec:discuss}
% %It is confirmed that the high-frequency shape can be recovered by learning with synthetic shading images, however, 
% It is confirmed that there remains severe ambiguity in our method, \ie, scale ambiguity including negative direction. %remains, which is our important future research.
% %One is scale and the other 
% %On the other hand, the scale of the restored shape is different from the real scale.
% As shown in \figref{failure_case}(a)(b), a convexity of the shape is inversely recovered.
% %to opposite direction.
% %to reality is inferred in several cases.
% The reason can be explained by bas-relief ambiguity, because the simplified rendered images with our method do not reproduce the effects of inter-reflection, ambient occlusion nor global illumination effect, which are important to decide a concave-convex ambiguity as shown in \figref{failure_case}(c)(d) for real example.
% %at the small concavity that should actually exist.

% \begin{figure}[t]
%     \centering
%     \subfigure[]{\includegraphics[width=1\linewidth]{figs/Result/failure_case.pdf}}
%     \subfigure[]{\includegraphics[width=0.4\linewidth]{figs/discussion/topview_cocave.jpg}}
%     \subfigure[]{\includegraphics[width=0.5\linewidth]{figs/discussion/sideview_cocave.jpg}}
%     \caption{Failure case. (a) error map between reconstructed shape and ground truth, (b) close-up view of 3D shapes, (c) example of bas-relief ambiguity, and (d) side view of (c).}
%     \label{fig:failure_case}
% \end{figure}

% \begin{figure}[tb]
%     \centering
%     \vspace{-0.2cm}
%     \begin{tabular}{ccc}
%     \includegraphics[width=1 \linewidth]{figs/Result/failure_case.pdf} &
%     \includegraphics[width=0.4 \linewidth]{figs/discussion/topview_cocave.jpg}&
%     \includegraphics[width=0.4 \linewidth]{figs/discussion/sideview_cocave.jpg}\\
%     (a) \hspace{2.5cm} (b) & (c) & (d)\\
%     \end{tabular}
% %    \vspace{0.1cm}
%     \caption{Failure case. (a) error map between reconstructed shape and ground truth, (b) close-up view of 3D shapes, (c) example of bas-relief ambiguity, and (d) side view of (c).}
%     \label{fig:failure_case}
% %    \vspace{-0.2cm}
% \end{figure}

==> tex/introduction.tex <==
\section{Introduction} \label{sec:intro}
%\knote{短すぎる}
Importance of active stereo method based on structured-light is 
increasing because of its simple system configuration and potential of 
high accuracy shape reconstruction. Gray-code and phase-shift, which are known 
as temporal coding methods, are typical implementation and 
have been widely used so far. Since those techniques
%gray-code and phase-shift 
require multiple patterns to identify the
pixel location, fast moving object cannot be captured.
To compensate the problem, oneshot scanning methods draw a wide attention, which is based on sparse structured light comprising
codes for identification in the single pattern, achieving shape reconstruction 
from one or only a few pattern projection.  %to reconstruct the shape,
%they are 
%and applicable to measurement of dynamic objects.
A common problem of the sparse structured light methods
is that the resolution of reconstruction is much lower than temporal coding 
method, specifically they can only recover the shape around the pattern region, 
which is sparse. 
%area.
%Since it is not able to find corresponding points in such area, the 
%shape is not reconstructed by triangulation.

In this paper, we tackle with this problem to recover dense and high-frequency 
shapes by using color information, which is captured by 
oneshot RGB-D sensor based on structured light and single camera.
%together with depth information.
%reconstruction, including patternless area by utilizing lattice
%structured light [1].
In previous methods, which usually employ
interpolation by median filter, Gabor filter or moving average, the regions which have no pattern projection are reconstructed as a low-frequency shapes, 
\ie, smooth/flat surfaces, even if the surface has high frequency shapes.
%, i.e. the surface with small bumps.
With our technique, {\it shading information} of
%in order to reconstruct the dense shape in the
such no pattern projected regions is analyzed and high-frequency shapes are 
recovered from oneshot (single) color image. % from single image.
%by using deep neural network which is expected to mimic the shape from 
%shading techniques from single image. 
Since multiple images 
with different lighting positions are usually required for shape from shading 
techniques, it is theoretically impossible to recover shape only from single image. For 
solution, we propose a learning based approach to recover the shapes upto scale 
from 
single image. In addition, to overcome the problem of preparing 
sufficient amount of data for training, we propose a domain adaptation method 
where new training data set are generated by computer graphics technique
%augmentation method 
using parametric representation of high-frequency shapes. 
% Those synthesized shapes are efficiently used to recover real 
% object based on transfer learning. 
Those synthesized shapes are efficiently used to learn high-frequency shapes and a few real data are used to adapt our model to real environment.
Experimental results are shown to 
confirm the effectiveness of the proposed method compared  with previous 
method, \eg, shape super-resolution techniques. 
%\knote{Please confirm the followings are surely discussed in the experimental section.} One interesting finding through the experiment is that convex/concave ambiguity problem can only be solved after fine-tuning using real data set,
%after transfer learning, 
%which is discussed in the experimental section.
%%
Our contributions are threefold:
\begin{itemize}
  \setlength{\parskip}{0cm} % 段落間
  \setlength{\itemsep}{0cm} % 項目間
\item Dense and high-frequency shape reconstruction method
using convolutional neural network (CNN), whose input is
a single shading image and a single sparse depth image, is proposed.
\item Efficient domain adaptation %data augmentation
 method using huge amount of computationally generated images based on parametric 
representation of high-frequency shapes is proposed, which is futher improved by 
		  fine turing technique using realdata.
%efficiently used for transfer learning.
\item It is shown that the proposed network is able to reconstruct dense and 
high-frequency shapes using real data set, comparing with previous methods.
\end{itemize}

==> tex/method.tex <==
\section{Shape recovery from shading information} \label{sec:recovery}
%\subsection{Overview}


\subsection{Algorithm overview}

\begin{figure}[t]
    \centering
%\vspace{2.5cm}
%\knote{Need blcok diagram or some figure here!!}
%\vspace{2.5cm}
   \includegraphics[width=1.0\linewidth]{figs/block_diagram-eps-converted-to.pdf}
%   \includegraphics[width=1.0\linewidth]{figs/block_diagram.eps}
    \caption{Algrithm overview.}
    \label{fig:algorithm}
\end{figure}

Our method reconstructs the high-frequency shape by adding a high-frequency component estimated from shading to the measured low-frequency shape.
First, we measure the low-frequency shape of the object and the shading image under fixed illumination.
For low-frequency shapes, a one-shot measurement with a projector and camera system~\cite{Furukawa2016} is used, but the shape measurement method in our framework is not limited to this technique.
Next, the low-frequency shape and shading images are input into the CNN to reconstruct the high-frequency shape.
Learning the shading of high-frequency shapes requires a lot of training data, however the measurement of many variations of objects is time consuming and the measurement of high-frequency shapes that are ground truth is also difficult.
Therefore, we construct a synthetic dataset of shading images by computer graphics and perform transfer learning.
The construction of the synthetic dataset is discussed in detail in \secref{synthetic}.


\subsection{System configuration and inital data acquisition}

%\subsection{Low-frequency shape measurement using sparse structured light}

One-shot measurement using a projector and camera system with a grid pattern~\cite{Furukawa2016} is used as a method to measure the low-frequency shape.
Setup is shown in \figref{gapreconst}(a).
The pattern projected by the projector consists of a sparse grid pattern (\figref{gapreconst}(b)), with codes embedded as a positional relationship between adjacent grid points (\figref{gapreconst}(c)).
By identifying grid points using codes, the corresponding points to the image captured by the camera are detected, and the distances are calculated by triangulation.
With the grid pattern, only the shapes on the lines that make up the pattern can be measured.
We obtain low-frequency shapes by interpolating the sparse shapes with the Radial Basis Function (RBF).

\begin{figure}[t]
    \centering
%   \includegraphics[width=0.7\linewidth]{figs/cap_scene_dot_line.eps}
   \includegraphics[width=0.8\linewidth]{figs/cap_scene_dot_line-eps-converted-to.pdf}
    \caption{System configuration of the oneshot system using dot and line pattern which is robust, but achieves only sparse reconstruction.}
%
%
    \subfigure[]{\includegraphics[width=0.6\linewidth]{figs/Setup/exp-setup.jpg}}
    \\
    \subfigure[]{\includegraphics[width=0.45\linewidth]{figs/GapReconst/grid_pattern.png}}
    \subfigure[]{\includegraphics[width=0.45\linewidth]{figs/GapReconst/gap_code.png}}
    \caption{(a) Setup of the measurement. (b) To measure the low-frequency shape, a sparse grid pattern is projected onto the object. (c) The grid points are decoded into different codes depending on their connection to their neighbors.}
    \label{fig:gapreconst}
\end{figure}

\section{Implementation} 
%\section{Shape recovery from shading information} \label{sec:recovery}
%\label{sec:recovery}


\subsection{High-frequency shape recovery from shading information using CNN}

Using the fact that the shading changes depending on the normal of the object's surface and the direction of the light source, we recover the lost high-frequency shape by using high-resolution shading images.

Since the shading does not imply an absolute depth, only the high-frequency shape, i.e., a normal direction is estimated from the shading in addition to the measured low-frequency shape.

In order to relax the measurement conditions, we fix the light source position to a single position and use only a single shading image.
In order to analytically recover the shape from the shadows, multiple images with different light source positions are required.
Our machine learning approach recovers shape from a single shading image by learning the shape and corresponding shading in the lighting environment for a sufficient sample.
To recover high-frequency components from shading images using CNN.

The proposed network takes three images as input: a shading image, a low-frequency depth image, and a pattern projection image.
The shading is the main clue for estimating the high-frequency shape.
Low-frequency depth images are expected to give additional clue to the low-frequency normal direction, and pattern projection images are expected to help in estimating the pixel-by-pixel confidence of low-frequency depth images.
The output of the network is the high-frequency shape and during training is the difference between the low-frequency shape and the ground truth.

%\subsection{Network structure}

We employ U-Net~\cite{Ronneberger2015} structure to learn relationship between a local feature of the shading and the shape.
Since U-Net is composed of pooling layers and up-sampling layers and skip connection between these layers, it is able to retain the local and global information.
Our network structure is shown in \figref{network_structure}.
After input is converted into 32-dimensional feature by multiple convolutions, low-resolution feature is extracted by max-pooling layer, then, it is converted into a high-resolution feature by deconvolution.
Due to skip connections between pooling layers and up-sampling layers, the output reflects both low-resolution and high-resolution features.

The three images, the shading image, the low-frequency depth image, and the pattern projection image, are concatenated and input into the network as three channels, and the high-frequency component of the shape is output.
Projected images are normalized to a maximum value of 1, while shading images are normalized to a mean of 0 and a variance of 1.
We set the kernel size to 3 and the number of layers to 3.
For loss function, We compute Root Mean Squared Error (RMSE) for the area where the low-frequency depth is available.
In order to reduce the memory usage, the input is divided into small patches in the training stage, as $1200\times1200$ original input images are divided into $120\times120$ small patches.
In the inference stage, the input image is processed in the original resolution.
The training is stopped at the epoch where the validation loss value is at its minimum.

\begin{figure}[t]
    \centering
    \includegraphics[width=1 \linewidth]{figs/Network/network-structure.pdf}
    \caption{The proposed network for shading learning is based on the U-Net structure.}
    \label{fig:network_structure}
\end{figure}


%\section{Transfer learning with synthesized shading images} \label{sec:transfer}
%\subsection{Data augmentation using synthesized data}
\subsection{Domain adaptation using synthesized data} \label{sec:synthetic}

The proposed network requires a ground truth of high-frequency shape as input.
In order to estimate the shading of various high-frequency shapes, it is necessary to measure many variations of objects in many poses, and the number of measurements is huge.
In addition, high-frequency shapes are difficult to measure, and accurate shapes may not be obtained.
Therefore, we propose a domain adaptation method for measuring objects in the real environment by learning a dataset by augmenting it with synthetic images generated by rendering graphics.


\subsubsection{Generation of synthesized data}
Since we intend to learn the shading of shapes, we need to create a variety of shapes and generate shading images.
First, to reproduce various high-frequency shapes, an approach that utilizes a dataset of public 3D shapes is considered.
However, high-resolution 3D shape, including high-frequency shape, has a large data size.
Furthermore, the distribution of normals included in the shape is expected to be biased, and if the shape to be measured is significantly different from the data set, the recovery accuracy is should be reduced.

We generate shapes procedurally to cover many shapes and to make it easier to fine-tune the parameters for the learning.
To generate procedural shapes, we adopt harmonic functions.
First, a two-dimensional height map is generated by the following function,
\begin{equation}
	I(x, y)= \sum_{i=0}^N \alpha_i \cos \left( 2 \pi x^{\prime} \lambda_i + \psi_i \right), x^{\prime} = x \cos \theta_i + y \sin \theta_i,
\end{equation}
where $\alpha$ is coefficient, $\lambda$ is wavelength, and $\psi$ is phase, that are randomly chosen, and $N$ is the number of the basis.
After the height map is generated, the mesh for rendering is generated.

Next, we will explain the rendering.
To reproduce the measurement environment, the scene is set up with the same intrinsic camera matrix, intrinsic projector matrix, and relative pose as the real environment setup.
The camera and projector assumed a perspective projection model.
In order to reproduce the physically correct appearance, the rendering can be performed by path tracing.
While Monte Carlo-based path tracing can reproduce the effects of inter-reflections and global illumination, it is found that it requires a lot of time for rendering and sampling noise negatively affects the learning results.
Therefore, we generate shading images by rasterization.
Rendering by rasterization renders fast and the direct reflection is accurately rendered without sampling noise generated.
The distance and projection images are also generated by rasterization.
We implement the renderer by modifying the Open-GL based \textit{PyRender}\cite{Pyrender}.

An example of a shading image with regularly varying $\theta$ and $\lambda$ is shown in \figref{synth_param}.
Note that these two parameters are a subset of the wide all-parameter space, but they generate a large number of variations.
In this paper, we manually adjust the parameters to obtain a shape close to the real object.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9 \linewidth]{figs/Synthesize/synth_params.pdf}
    \caption{Examples of shading image of the shape when varying $\theta$ and $\lambda$, which generate many variations of the shape, even for the two parameters.}
    \label{fig:synth_param}
\end{figure}


\subsubsection{Training and Fine-tune using real-world data}
The network weights of the model learned from the synthesized images do not work well for real-world input with different image features because the weights are adapted only to the domain of the trained domain.
In order to support real-world input, we additionally train and fine-tune the network model.
The network is expected to learn feature extraction from real-world images and encoding to depth.
To perform a fine-tune, the network input is only a few real-world data, and the weights of all layers are updated.
The training is stopped when the value of validation loss is at a minimum.


==> tex/recovery_shading.tex <==
\section{Shape recovery from shading information} \label{sec:recovery}
\subsection{Overview}

Our method reconstructs the high-frequency shape by adding a high-frequency component estimated from shading to the measured low-frequency shape.
First, we measure the low-frequency shape of the object and the shading image under fixed illumination.
For low-frequency shapes, a one-shot measurement with a projector and camera system~\cite{Furukawa2016} is used, but the shape measurement method in our framework is not limited to this technique.
Next, the low-frequency shape and shading images are input into the CNN to reconstruct the high-frequency shape.
Learning the shading of high-frequency shapes requires a lot of training data, however the measurement of many variations of objects is time consuming and the measurement of high-frequency shapes that are ground truth is also difficult.
Therefore, we construct a synthetic dataset of shading images by computer graphics and perform transfer learning.
The construction of the synthetic dataset is discussed in detail in \secref{synthetic}.

\subsection{Low-frequency shape measurement using sparse structured light}

One-shot measurement using a projector and camera system with a grid pattern~\cite{Furukawa2016} is used as a method to measure the low-frequency shape.
Setup is shown in \figref{gapreconst}(a).
The pattern projected by the projector consists of a sparse grid pattern (\figref{gapreconst}(b)), with codes embedded as a positional relationship between adjacent grid points (\figref{gapreconst}(c)).
By identifying grid points using codes, the corresponding points to the image captured by the camera are detected, and the distances are calculated by triangulation.
With the grid pattern, only the shapes on the lines that make up the pattern can be measured.
We obtain low-frequency shapes by interpolating the sparse shapes with the Radial Basis Function (RBF).

\begin{figure}[t]
    \centering
    \subfigure[]{\includegraphics[width=0.36\linewidth]{figs/Setup/exp-setup.jpg}}
    \subfigure[]{\includegraphics[width=0.27\linewidth]{figs/GapReconst/grid_pattern.png}}
    \subfigure[]{\includegraphics[width=0.27\linewidth]{figs/GapReconst/gap_code.png}}
    \caption{(a) Setup of the measurement. (b) To measure the low-frequency shape, a sparse grid pattern is projected onto the object. (c) The grid points are decoded into different codes depending on their connection to their neighbors.}
    \label{fig:gapreconst}
\end{figure}

\subsection{High-frequency shape recovery from shading information}

Using the fact that the shading changes depending on the normal of the object's surface and the direction of the light source, we recover the lost high-frequency shape by using high-resolution shading images.

Since the shading is not an absolute depth but a shape, i.e., a normal direction, only the high-frequency component is estimated from the shading in addition to the measured low-frequency shape.

In order to relax the measurement conditions, we fix the light source position to a single position and use only a single shading image.
In order to analytically recover the shape from the shadows, multiple images with different light source positions are required.
Our machine learning approach recovers shape from a single shading image by learning the shape and corresponding shading in the lighting environment for a sufficient sample.
To recover high-frequency components from shading images using CNN.

The proposed network takes three images as input: a shading image, a low-frequency depth image, and a pattern projection image.
The shading is the main clue for estimating the high-frequency shape.
Low-frequency depth images are expected to remove scale ambiguity according to depth, and pattern projection images are expected to help in estimating the pixel-by-pixel confidence of low-frequency depth images.
The output of the network is the high-frequency shape and during training is the difference between the low-frequency shape and the ground truth.

\subsection{Network structure}

We employ U-Net~\cite{Ronneberger2015} structure to learn relationship between a local feature of the shading and the shape.
Since U-Net is composed of pooling layers and up-sampling layers and skip connection between these layers, it is able to retain the local and global information.
Our network structure is shown in \figref{fig:network_structure}.
After input is converted into 32-dimensional feature by multiple convolutions, low-resolution feature is extracted by max-pooling layer, then, it is converted into a high-resolution feature by deconvolution.
Due to skip connections between pooling layers and up-sampling layers, the output reflects both low-resolution and high-resolution features.

The three images, the shading image, the low-frequency distance image, and the pattern projection image, are concatenated and input into the network as three channels, and the high-frequency component of the shape is output.
We set the kernel size to 3 and the number of layers to 3.
For loss function, We compute root mean squared error for the area where the interpolated depth is available.
In order to reduce the memory usage, the input is divided into small patches.
We divide $1200\times1200$ original input images into $120\times120$ small patches.
Projected images are normalized to a maximum value of 1, while shaded images are normalized to a mean of 0 and a variance of 1.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6 \linewidth]{figs/Network/network-structure.pdf}
    \caption{The proposed network for shading learning is based on the U-Net structure.}
    \label{fig:network_structure}
\end{figure}


==> tex/related_work.tex <==
\section{Related work} \label{sec:related}
\subsection{Shape from shading and photometric stereo}
Shapes from shading have been studied for a long time~\cite{Horn1974, Zhang1999}.
Photometric stereo, which uses shading to compute the normal distribution analytically, has been widely studied since it was proposed by Woodham~\cite{Woodham1980}.
For Lambertian photometric stereo for diffuse surfaces, three light sources are required.
Recently, some machine learning-based methods have been proposed, for example, Ikehata has proposed a CNN for photometric stereo in the presence of inter-reflections~\cite{Ikehata2018}.
%%
It is known as bas-relief ambiguity~\cite{belhumeur1999bas}, in which the shape cannot be uniquely determined from an image taken in a single light source environment.
Barron and Malik recover the most likely shape, illumination, and reflectance from a single shading image by imposing a strong prior on the object properties~\cite{Barron2015}.
Henderson and Ferrari propose a method to estimate shape, pose, and shading from a single image by generating a shape model and evaluating the shading of the rendered image~\cite{Henderson2019}.

\subsection{Super-resolution of 3-D shape}
The use of high-resolution RGB images has been studied as a clue to increase the resolution of low-resolution shapes obtained by RGB-D cameras.
The method to generate a high-resolution distance image from low-resolution distance images and high-resolution RGB images is called guided super-resolution.
Barron \etal proposed a method to propagate the depth using the RGB image as a guide using the fast bilateral filter~\cite{Barron2016}. 
Lutio \etal have achieved a pixel-to-pixel mapping using a multi-layer perceptron~\cite{Lutio2019}.
While these are unsupervised methods, a learning approach has been proposed by Hui \etal~\cite{Hui16}.
In this method, a CNN called a multi-scale guided network extracts features of different scales by an encoder and upsamples them by a decoder.
%%
In these methods, RGB images taken passively are taken for guides, while the proposed method uses the shading image taken under artificial illumination to be guided by shading.

\subsection{Synthetic training data}
It is important to prepare a sufficient amount of training datasets for machine learning, especially for methods using deep learning.
However, the data required for the technique, e.g., data measured or annotated in a particular system, are often not sufficiently present.
In addition, it is sometimes difficult to measure in a real-world environment.
In order to solve this problem, the method of constructing and learning data sets by data synthesis has become an important research topic in recent years.
%%
Weinmann et al. used synthesized data with a bidirectional texture function for learning the material classification~\cite{Weinmann2014}.
Experiments have shown that classification is possible in this task by training on images rendered with the same setup as in the real environment.
Dosovitskiy et al. have created a synthetic image dataset for learning optical flow by CNN~\cite{Dosovitskiy2015}.
Even though it consists of an unrealistic scene of a chair in flight, it achieves high estimation accuracy in a dataset measured in the real environment.
Using synthesized data for photometric stereo learning, Ikehata constructed a concave shaped dataset with complex shading, which is difficult to collect in large numbers by measurement, and showed that the real dataset can be reconstructed by the trained model~\cite{Ikehata2018}.

==> tex/transfer_learning.tex <==
\section{Transfer learning with synthesized shading images} \label{sec:transfer}
\subsection{Data augmentation using synthesized data}
The proposed network requires a ground truth of high-frequency shape as input.
In order to estimate the shading of various high-frequency shapes, it is necessary to measure many variations of objects in many poses, and the number of measurements is huge.
In addition, high-frequency shapes are difficult to measure, and accurate shapes may not be obtained.
Therefore, we propose a transfer learning method for measuring objects in the real environment by learning a dataset by augmenting it with synthetic images generated by rendering graphics.


\subsection{Generation of synthesized data}
Since we intend to learn the shading of shapes, we need to create a variety of shapes and generate shading images.
First, to reproduce various high-frequency shapes, an approach that utilizes a dataset of public 3D shapes is considered.
However, high-resolution 3D shape, including high-frequency shape, has a large data size.
Furthermore, the distribution of normals included in the shape is expected to be biased, and if the shape to be measured is significantly different from the data set, the recovery accuracy is should be reduced.

We generate shapes procedurally to cover many shapes and to make it easier to fine-tune the parameters for the learning.
To generate procedural shapes, we adopt harmonic functions.
First, a two-dimensional height map is generated by the following function,
\begin{equation}
	I(x, y)= \sum_{i=0}^N \alpha_i \cos \left( 2 \pi x^{\prime} \lambda_i + \psi_i \right), x^{\prime} = x \cos \theta_i + y \sin \theta_i,
\end{equation}
where $\alpha$ is coefficient, $\lambda$ is wavelength, and $\psi$ is phase, that are randomly chosen, and $N$ is the number of the basis.
After the height map is generated, the mesh for rendering is generated.

Next, we will explain the rendering.
To reproduce the measurement environment, the scene is set up with the same intrinsic camera matrix, intrinsic projector matrix, and relative pose as the real environment setup.
The camera and projector assumed a perspective projection model.
In order to reproduce the physically correct appearance, the rendering can be performed by path tracing.
While Monte Carlo-based path tracing can reproduce the effects of inter-reflections and global illumination, it is found that it requires a lot of time for rendering and sampling noise negatively affects the learning results.
Therefore, we generate shading images by rasterization.
Rendering by rasterization renders the directly reflected light accurately and fast so that shading can be reproduced and sampling noise is not generated.
The distance and projection images are also generated by rasterization.
We implement the renderer by modifying the Open-GL based renderer pyrender\cite{Pyrender}.

An example of a shading image with regularly varying $\theta$ and $\lambda$ is shown in \figref{synth_param}.
Note that these two parameters are a subset of the wide all-parameter space, but they generate a large number of variations.
In this paper, we manually adjust the parameters to obtain a shape close to the real object.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5 \linewidth]{figs/Synthesize/synth_params.pdf}
    \caption{Examples of shading image of the shape when varying $\theta$ and $\lambda$, which generate many variations of the shape, even for the two parameters.}
    \label{fig:synth_param}
\end{figure}

\subsection{Training}
Of the 200 simulation data, 40 data were used as test data, and 48 of the remaining 160, or 30\% of the data, were used as validation data, resulting in 92 pieces of training data.
The $1200\times1200$ resolution data is clipped into $120\times120$ resolution patches and entered into the network.
The model was trained at 400 epochs and evaluated with the model at the point of lowest validation loss.

In addition to the synthetic data, we prepared 6 types of real objects taken in the real environment: cardboards with three different high-frequency shapes and the other three objects with more complex surface shapes.
Of the three cardboards A, B, and C, 8 data taken at A are used as fine-tuning data and 16 data taken at B and C are used as test data.
After training on simulation data, the model was fine-tuned on data taken on cardboard A in the real environment.
